Federated Learning over Next-Generation Ethernet Passive Optical Networks

Federated Learning (FL) is a distributed machine learning (ML) type of processing that preserves the privacy of user data, sharing only the parameters of ML models with a common server. The processing of FL requires specific latency and bandwidth demands that need to be fulfilled by the operation of the communication network. This paper introduces a Dynamic Wavelength and Bandwidth Allocation algorithm for Quality of Service (QoS) provisioning for FL traffic over 50 Gb/s Ethernet Passive Optical Networks. The proposed algorithm prioritizes FL traffic and reduces the delay of FL and delay-critical applications supported on the same infrastructure.

==> algorithm_coop_2.tex <==
\begin{algorithm}[!t]

 %\small

    \caption{\coopGSIPACT DBA Algorithm}
    \label{alg:gs-ipact}
\SetAlgoLined


\SetKwInput{KwIni}{}
\KwIni{$\mathcal{R}_{l} \leftarrow \emptyset, \forall l \in \mathcal{G}$}
\KwIni{$\mathcal{R}_{k} \leftarrow \emptyset, \forall k \in \mathcal{M}$}

    \For{each received report R from \ac{ONU} i in cycle j}{ 



        \eIf{ONU $i \in \mathcal{O}_{T}$}{
        
            Send $Gate^j_{i}$ according to  \ac{IPACT} limited policy \cite{IPACT}
            
            SaveReportCoop()
          
            
            
        }{%else
    
            $\mathcal{R}_{k} = \mathcal{R}_{k} \cup \{R\}$

            \If{ $\left\vert{\mathcal{R}_{k}}\right\vert$ = $\left\vert\mathcal{O}_{k}\right\vert$}
            {%else
                
                %$\mathcal{S}_{s} = \mathcal{S}_{s} \cup \{R.subgroup()\}$
                
                BulkGrantGenerator()
            } 
             
       
       }
       
       
            \If{ $\left\vert{\mathcal{R}_{l}}\right\vert$ = $\left\vert\mathcal{O}_{l}\right\vert$}
            {%else
                MultiThreadCoop()
            }
       
        }
       
    

       %\mathcal{R}_k \leftarrow \emptyset
      


  \SetKwFunction{FMain}{\textbf{BulkGrantGenerator}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{

      
    \For{each report $R_i \in \mathcal{R}_{k}$}{ 

       
        Send $Gate^j_{i}$ according to  \GSIPACT excess distribution policy \cite{MOS-IPACT}
        
        SaveReportCoop()
      
             
    }
     
     $ \mathcal{R}_{k} \leftarrow \emptyset$
        

 }
\textbf{end}

  \SetKwFunction{FMain}{\textbf{SaveReportCoop}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{

      
    \If{ONU $i \in \mathcal{O}_{l}$}
    {   
        
        
        \eIf{$R_i  >  W^{granted}_{i}   $}
         {%else
         $\mathcal{R}_{l} = \mathcal{R}_{l} \cup W^{extra}_{i}$
         }{
          $\mathcal{R}_{l} = \mathcal{R}_{l} \cup 0$
         }
    }
        

 }
\textbf{end}


\SetKwFunction{FMain}{\textbf{MultiThreadCoop}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{

     \For{each report $R_i \in \mathcal{R}_{l}$}{ 
     
     Calculate $W^{threadCoop}_{i}$ according $(2)$
        
        \If{$W^{threadCoop}_{i}>0$}
        {   
         
          Calculate $t_{txStart}$  
        
          $Gate^j_{i}\leftarrow$\hspace{0.1cm}$(W^{threadCoop}_{i},t_{txStart})$
                           
          Send $Gate^{j}_{i}$

        }
     
     
     }


 }
\textbf{end}


\end{algorithm}

==> mBS.tex <==
\begin{algorithm}[!t]

 %\small

    \caption{\BS \ac{DWBA} Algorithm}
    \label{alg:gs-ipact}
\SetAlgoLined


\SetKwInput{KwIni}{}
% \KwIni{$\mathcal{R}_{l} \leftarrow \emptyset, \forall l \in \mathcal{G}$}
\KwIni{$\mathcal{R}_{i} \leftarrow \emptyset, \forall i \in \mathcal{O}$}

    \For{each received report R from \ac{ONU} i in cycle j}{ 

        \If{ONU $i \in \mathcal{O}$}{
        
        
            \eIf{ $\left\vert{\mathcal{R}_{fl}}\right\vert$ > $0$}
            {%else
                
                 $Granted^{fl}_{i}  \leftarrow \hspace{0.1cm}  BandwidthSlicing()$
                
              
            
            }{
            
              $Granted^{fl}_{i} \leftarrow \hspace{0.1cm}  \left\big(0,0,0\right\big)$
            
            } 
        
             $Granted^{fl}_{i}  \leftarrow \hspace{0.1cm}  BandwidthAllocation()$
            
            $Gate^{j}_{i} =  (Granted^{ds}_{i},  Granted^{fl}_{i})$
            
            
            
            
            Send $Gate^{j}_{i}$
            

        }
       
        }
       %\mathcal{R}_k \leftarrow \emptyset
   
  \SetKwFunction{FMain}{\textbf{BandwidthSlicing}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{


         $w^{fl}_{i} = min(\left\vert{\mathcal{R}_{fl}}\right\vert$,  $\theta\cdot Z $)

        Calculate $f^{fl}_{i}$ based on \ac{TWDM}-scheduler 
    
        Calculate  $t^{fl}_{i}$
    
    %   \textbf{return}  $\left\big(f^{fl}_{i},w^{fl}_{i},t^{fl}_{i}\right\big)$
 }
\textbf{\textbf{return}  $\left\big(f^{fl}_{i},w^{fl}_{i},t^{fl}_{i}\right\big)$}

  

  \SetKwFunction{FMain}{\textbf{BandwidthAllocation}}
    \SetKwProg{Fn}{}{}{}
    \Fn{\FMain{}}{


        $w^{ds}_{i} = min(\left\vert{\mathcal{R}_{ds}}\right\vert$, w^{max}_i)
        %calculate w according to the limited policy
            
        Calculate  $f^{ds}_{i}$ based on \ac{TWDM}-scheduler 
  
        Calculate  $t^{ds}_{i}$
    
    %   \textbf{return}  $\left\big(f^{ds}_{i},w^{ds}_{i},t^{ds}_{i}\right\big)$
 }
\textbf{\textbf{return}  $\left\big(f^{ds}_{i},w^{ds}_{i},t^{ds}_{i}\right\big)$}

\end{algorithm}

==> proposal_test.tex <==
\section{Group-\ac{SLA} \ac{DBA} Scheme for EPON Networks}
\label{sec:proposal}

This section introduces a \ac{DBA} algorithm for supporting group-SLAs in EPON networks called \GSIPACT. It is based on the widely used \ac{IPACT} algorithm \cite{Kramer_2012_983911} to enable a group assured bandwidth. \ac{IPACT} uses an interleaved polling approach where the next ONU is polled before the transmission from the previous one has arrived, this achieve the statistical multiplexing gain in relation with \ac{TMDA}. In this scheme the \ac{OLT} could execute various politics (i.e. gated, limited, elastic, linear credit, or constant credit) for define the assigned bandwidth. Furthermore, each \ac{ONU} have a \ac{SLA} which specifies the  minimum guaranteed bandwidth and the maximum windows size ($W_{max}$), thus the ONU gets a Gate to send as many bytes as it has requested, but no more than the limit ($W_{max}$). Finally, the adaptive cycle time is an important feature of \ac{IPACT}. Under heavy load conditions, the cycle length is equally to the maximum cycle time will result in increased delay for all the packets. Further, when there is no high traffic, the length cycle decreases will result in more bandwidth being wasted by guard times and signaling. 

Despite these features, the \ac{MNO}s with more than one \ac{ONU} in the same \ac{PON} can not used the statistical multiplexing properties between their \ac{ONU}s. In \GSIPACT, the interleaved polling is modified for wait the requests of all \ac{ONU}s that belong to the same SLA-group. Every time that arrive a Report, the conventional policies are applied for find the windows legacy length and ensure the guaranteed minimum bit rate. \GSIPACT do not send the Gates of the \ac{ONU}s-group until the arrive of all Reports. When arrive, the \ac{ONU}s are classified in underloaded and overloaded. Subsequently, it is calculated the excess total bandwidth from the underloaded \ac{ONU}s-group and the total bandwidth needed from the overloaded \ac{ONU}s-group. After this process, an algorithm (i.e DBA1, DBA2, DBA3, WDBA1 and WDBA2)  distribute the total excess  bandwidth between the overloaded \ac{ONU}s-group. Every overloaded \ac{ONU}  receive a portion of the total excess bandwidth called new length bandwidth. Finally the Gate will have a value equally to the legacy length plus the new length bandwidth. However, when a Report of a \ac{ONU} that do not belong to the group arrive, the \ac{OLT} execute the normal process with the \ac{IPACT} scheme. 


The Figure 1 represent the scheduling of the GS-IPACT scheme...

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{img/Diagramas/GS-IPACT}
    \label{fig:GS-IPACT}
   % }%\vspace*{-2.5em}
   \centering
    \caption{GS-IPACT scheduling}
\end{figure*}


\subsection{The scheme effect in the wasted}


\subsubsection{\ac{IPACT} Case} 
The Figure 2 represents the wasted caused by the \ac{IPACT} scheme...

The wasted for the IPACT scheme with excess distribution depend of the cycle length and the minimum RTT, as show the following formulas.



  \begin{equation} 
  Cycle = 1000  us \label{Ec:DBA4x}
  \centering 
  \end{equation}

  \begin{equation} 
  RTT = [100, 200] us \label{Ec:DBA4x}
  \centering 
  \end{equation}
  
   \begin{equation} 
  Wasted= [10, 20]\%
  \label{Ec:DBA2x}
  \centering 
  \end{equation}
  



 \subsubsection{GS-\ac{IPACT} case} 
 The figure 3 represents the wasted caused by the GS-\ac{IPACT} scheme.
 

 
 Para que no exista wasted se debe cumplir que:
 
  \begin{equation} 
  RTT > \sum_{i=1}^{C} (Wmax_i + GT_i) 
  \label{Ec:DBA3x}
  \centering 
  \end{equation}

Where $C$ represent the other \ac{ONU}s, that are not in the group.  

Si Wmax es igual a

 \begin{equation} 
  W_{max} = \frac{Cycle-nOnus*GT}{nOnus} = 30.25 us
  \label{Ec:DBA3x}
  \centering 
  \end{equation}


Thus the wasted is represented by the follow formula.

  \begin{equation} 
  Wasted[sec] = RTT - \sum_{i=1}^{C} (Wlength_i + GT_i) 
  \label{Ec:DBA3x}
  \centering 
  \end{equation}
  
  \begin{equation} 
  Wasted[\%] = \frac{(RTT - (nONUs - nONUsGroup)(\frac{Wlength*30.25}{100}+GT))*100}{Cycle length} 
  \label{Ec:DBA3x}
  \centering 
  \end{equation}
 


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{img/SchemeWasted/newWasted.pdf}
    \label{fig:GS-IPACT}
   % }%\vspace*{-2.5em}

    \caption{GS-IPACT scheme wasted}
\end{figure}



%follows the LTE specification and employs QoS-related metrics to prioritize users for scheduling.




==> related-work_backup.tex <==
\section{Related Work}
\label{sec:related-work}

    %This section reviews \ac{DBA} algorithms proposed for \ac{PON} networks, including both \ac{EPON} and \ac{GPON} technologies. We also include \ac{DBA} algorithms with excess bandwidth distribution policies.
    
    Several \ac{DBA} algorithms for \acp{EPON} have been proposed in the literature. These have been cataloged depending of three sub-problems[Michael Space]; grant scheduling framework, grant sizing policy, grant scheduling policy. The first one handle the Gate sent  decision triggered by a event.  The second one define the transmission windows length (slots) for each ONU. The third one determines the scheduling  order for the overloaded \acp{ONU} when a excess distribution bandwidth \ac{DBA} algorithm  is applies.  
    
    
    %Several \ac{DBA} algorithms for \acp{EPON} have been proposed in the literature.
    %Among them, 
    \ac{IPACT} \cite{Kramer_2002_983911} is one of the most important \acp{DBA}, since most of the existing algorithms are based on it. To achieve statistical multiplexing gain, \ac{IPACT} proposes an interleaved polling algorithm which gives transmission opportunities for each \ac{ONU} using a round robin mechanism. %IPACT is a online grant scheduling framework because when a Report arrives to \ac{OLT}, a Gate is immediately sending to \ac{ONU}.
    The granted transmission window depends on the grant sizing policy used by the service provider. 
    \ac{IPACT} defines four grant size policies called; fixed, closed, limited, and excess, being limited the most widely used. 
    In \ac{IPACT} with limited scheduling policy, each \ac{ONU} has a maximum window size $(W_{max})$, which is related to the guaranteed bandwidth specified in the assigned \ac{SLA}. IPACT is a online grant scheduling framework because when the \ac{OLT} receives a Report message $r$, a Gate message $g$ is sent to the \ac{ONU} containing the grant size, which is calculated as the minimum between the requested window $r$ and the maximum allowed window $(W_{max})$.
     
    %To improve the \ac{QoS} provisioning, \ac{IPACT} can combine inter-ONU scheduling (centralize technique) to allocate the transmission windows to each ONU and a  priority queuing intra-\ac{ONU} scheduling (distributed technique) to divide the bandwidth allocated by the OLT among the different traffics  based on priorities or \ac{CoS} in the \ac{ONU}. %Finally, the adaptive cycle time is an important feature of \ac{IPACT}. Under saturation conditions, the cycle length is equal to the maximum cycle time, which will result in increased delay for all the packets. Under light loads, the cycle length decreases, resulting in more bandwidth being wasted by guard times and signaling. 

    
    %\commentc{Put info about QoS Intelligentce: Centrilized vs QoS Distributed}   
    %the excess bandwidth algorithms in epon.
    % Novel bandwidth allocation with quota-based excess-distribution algorithm and wavelength assignment in multi-wavelength access network
     %The first grant sizing policy for excess bandwidth distribution was presented in \cite{EPON1}.%, where the wait-for-all-reports scheme was also introduced. 
    The excess distribution \ac{DBA} algorithms takes advantage of statistical multiplexing to improve the network performance in a heterogeneous traffic scenarios. Depending of their REPORT requests size and the guaranteed minimum bandwidth these algorithms divided the \acp{ONU} into underloaded and overloaded. Underloaded \acp{ONU} are whose that the REPORT requested size is equal or less than allow limited bandwidth ($R_i \leq W_{max}$), in the opposite case are know as overloaded \acp{ONU}, that is ($Ri>W_{max}$). The excess algorithms allow the use of unoccupied physical resources of underloaded \acp{ONU}, while is controlled the maximum cycle length.   
    
    The first grant sizing policy for excess bandwidth distribution was presented in \cite{EPON1}.  This policy, so called DBA1, %takes advantage of statistical multiplexing to improve the network performance in a heterogeneous traffic scenarios. % classes as defined in the \ac{DiffServ} framework. 
    multiplies the excess bandwidth for the ratio between the REPORT of the \ac{ONU} target and the Total REPORTS of the all overload ONUs, thus it allocates the excess bandwidth according to the total demand of the overloaded ONU. This approach do not give an equal piece of the excess bandwidth for the overloaded ONUs because the bandwidth allocated depend of the individual request size.

    %It multiplies the excess bandwidth for the ratio between the REPORT of the ONU target  and the Total REPORTS of the all overload ONUs.
    %The DBA policy allocates the excess bandwidth according to the demand of the overload \acp{ONU} following \autoref{Ec:DBA1}.
  
    %Where $C$ is the set of overloaded \acp{ONU} and $E_{total}$ the total excess bandwidth of all underloaded \acp{ONU} in a given scheduling cycle. This approach do not give an equal piece of the total excess because the excess allocated for a overloaded \ac{ONU} depend of the request size. 
    
    A simple excess distributed policy, so called DBA2, was propsoed in \cite{EPON2}. It divides the total excess bandwidth $E_{total}$ equally among the overloaded \acp{ONU}. This kind of policy is known as uncontrolled excess because the \ac{OLT} allocates uniformly the excess to all overloaded \acp{ONU} regardless of the requested bandwidth by each ONU.  %The uncontrolled excess method do not consider the request size from \acp{ONU}, 
    This means that a overloaded \ac{ONU} can receive a grant larger than its buffer size. To avoid this problem, a controlled excess bandwidth policy (so called DBA3) was proposed in \cite{EPON3}. This avoids wasting resources by granting bandwidth less than or equal to the required ($G_i \leq R_i$). 
    %In the uncontrolled excess bandwidth algorithm, the GATE for a overload \ac{ONU} always is equivalent to the sum between the maximum transmission window size and the excess bandwidth $(G_i = W_{max} + E_i)$. However, in DBA3 when the REPORT is less than this value $(W_{max} + E_i)$, the GATE is equal to the REPORT. This way the system do not assign more resources to a overload \ac{ONU} that it does not need it. 

    %In DBA1 and DBA2, there are no an excess controlled, it means a GATE for a overload \ac{ONU} always is equivalent to the sum between the maximum transmission window size and the excess bandwidth $(G_i = W_{max} + E_i)$. However, in DBA3 when the REPORT is less than this value $(W_{max} + E_i)$, the GATE is equal to the REPORT. This way the system do not assign more resources to a overload \ac{ONU} that it does not need it. 

    %This approach gives an equal piece of the total excess for all ONUs, implying fairness.

    In \ac{EPON} network coexist several services, thus the $W_{max}$ could be different for all \acp{ONU}. The DBA1 and DBA3 algorithm, distributed the bandwidth only using the REPORT.  The problem with this approaches it that they assume the all ONUs are in the equal conditions. In a unbalanced scenario in which the ONU have difference guaranteed bit rates, the algorithms before mentioned produce unfairness. Other approach called WDBA was proposed in \cite{EPON4}. This algorithm realize a better fairness bandwidth distribution, due to use  of the bandwidth excess required $(B_{req} = Ri - W_{max})$ instead of just the REPORT. If is applies the controlled excess method, it leads a new algorithm called WDBA1 \cite{EPON2}. 

%########################################################################
% GIANT
%########################################################################

    %put here the references to the two alvaro's papers 
    On the other hand, \ac{GIANT} is a well known \ac{DBA} algorithm for \ac{XGPON} \cite{Leligou_JCS2006_DAC:DAC761} that defines four type of bandwidths, namely, fixed, assured, non-assured and best-effort bandwidth. Alvarez \etal \cite{Pedro_NOC2014} \cite{Alvarez_JOCN2016-7444558} extends this algorithm to be used in \ac{XGPON}-based backhauling scenarios by introducing the \ac{gGIANT} algorithm. %. By adding a fifth type of bandwidth called group assured, \ac{gGIANT} allows 
    This algorithm shares the assured bandwidth among multiple \acp{ONU} that serve base stations belonging to the same operator. The authors show the benefits of sharing the assured bandwidth among a group of base stations. Both algorithms, however, are based on the concept of centralized \ac{QoS} intelligence \cite{Stribling_CM2012_SIEPON_6295722}, in which the \ac{OLT} is the responsible for the \ac{QoS} provisioning of the individual queues at the \ac{ONU}. This is optimal for small business or individual users but not for users with multiple connections at each \ac{ONU} as in the mobile backhauling use case. 
    
    
    The \ac{GPON} and \ac{EPON} technologies have a marked difference in the link layer architecture.  \ac{GPON} offers complex \ac{MAC} layer based on the ATM protocol. Multiple protocols make it possible the support the Ethernet frames.  Logical connections called \acs{XGEM} ports are generated for each type of service offered in the network. In addition, the equipment in \ac{GPON} networks requires some conversions of protocols, segmentation and virtual channel termination.  In contrast, \ac{EPON} technology do not use logical connections for different type of services because uses a native \ac{MAC} layer to support any type of IP-based network service (i.e. VoIP, Data, Video) over Ethernet frames.
    
     %\ac{XGPON} has intrinsic features that make different of \ac{EPON}
     
    There are also differences in terms of efficiency, scope, bandwidth, cost per user, management, protection, among others. EPON technology is characterized by extensive headers in the frames, which cause reduction in the payload bits and consequently low efficiency in contrast with \ac{GPON} solutions.  GPON is more flexible in therm of offered bandwidth, as it allows a asymmetric bit rates. The two technologies are focused in the access network, while GPON allows the vendor to set the rates taking into account the actual and actual needs, this mechanism that can not be realized in EPON networks.
    .....
    aun falta corregir arriba y terminar
    
    %\ac{GPON} have logical connections in the upstream and downstream direction called \acs{XGEM} ports to differentiate services which are established between \ac{OLT} and \ac{ONU}. Logical connections can also be grouped into \acp{T-CONT}. In this way, different levels of \ac{QoS} to different services belonging to a \ac{ONU} are enabled 
    
     %\ac{GPON}  must be added layers in the protocol to give the normal IP services
    
    
     In \ac{gGIANT}, a group of \acp{T-CONT} into a single logical connection provide service to groups of \acp{ONU} called \ac{gT-CONT}%, which is identified by the  \ac{gAllocId}. 
     It means that some  \acp{T-CONT} of the same \ac{ONU} could be in different \ac{gT-CONT}. 
       
     because the \ac{ONU} realize the individual intra-scheduling for different type of traffic based on priorities and send just a packet with a size defined by the \ac{OLT}.
     
     
    In summary, none of the above-reviewed \ac{EPON} \ac{DBA} schemes support group-\ac{SLA}. Even though there exists a \ac{XGPON} \ac{DBA} algorithm that supports group assured bandwidth, it cannot directly applied to \ac{EPON} networks. 
    First, \ac{XGPON} networks has a maximum cycle length of 125 us, whereas \ac{EPON} networks has a typical maximum cycle length value from 1 ms to 10 ms. This may help to improve the benefits the group \ac{SLA} concept brings since more bandwidth can be redistributed in a given scheduling period. Second, this paper works in a hierarchical DBA scheme in which the \ac{OLT} guarantees a given bandwidth while the intra-\ac{ONU} scheduler at the ONU is the responsible for providing the \ac{QoS} requirement of the different traffic \ac{ONU} flows. 

 Aumentar: las tecnologias compradas son diferentes longitud ciclo, estructura del header de las tramas de capa de enlace, el tamano de payload, la tasas bit, squedualing y ....

%%%####################################################################################
%\section{Related Work}
%\label{sec:related-work}
%%TODO Oscar
%    This section reviews \ac{DBA} algorithms proposed for \ac{PON} networks, including both \ac{EPON} and \ac{GPON} technologies. We divide this section in studies for the \ac{DBA} problem and those for excess distribution bandwidth. We conclude the section with a summary of the reviewed studies.
%\subsection{\acl{DBA} algorithms for \acp{PON}}
%\label{sec:dba-algorithm}
%%########################################################################
%% IPACT
%%########################################################################
%
%  
%    
%    %In the uplink direction \ac{EPON} employs the \ac{TDMA} technique to improves the performance compared with  the performance of the static bandwidth allocation.  Furthermore for the resource distribution and \ac{QoS} intelligence there are two well know techniques; centralized and  distributed. In the first one, the OLT is the only device that has global knowledge of the entire network for realize a centralize control and distributed the resources. In the second one, the \acp{ONU} perform the  scheduling, thus the \ac{OLT} is excluded from the implementation  of the resource allocation mechanism \cite{Sherif2004}.
%    
%     %In the uplink direction, \ac{EPON} can employs either a centralized or a distributed architecture to allocate resources and provide \ac{QoS}. In the former, the \ac{OLT} has global knowledge of the network, performing centralized control and resource allocation. In the latter, the OLT performs a per \ac{ONU} scheduling and each \ac{ONU} performs the intra-ONU scheduling \cite{Sherif2004}. %, thus the \ac{OLT} is excluded from the implementation  of the resource allocation mechanism . 
%     
%     Several \ac{DBA} algorithms for \acp{EPON} have been proposed in the literature. Among them, \ac{IPACT} \cite{Kramer_2002_983911} is one of the most important since most of the existing algorithms are based on it.
%     \ac{IPACT} proposes an interleaved polling algorithm to provide transmission opportunities for each \ac{ONU} using a round robin mechanism, achieving statistical multiplexing gain. 
%     The allocated time interval depends on the scheduling policy used by the network operator. 
%     \ac{IPACT} defines four policies called; fixed, closed, limited, and excess, being limited the most widely used. 
%     In \ac{IPACT} with limited scheduling policy, each \ac{ONU} has a maximum window size $(W_{max})$, which is related to the guaranteed bandwidth specified in the assigned \ac{SLA}. When the \ac{OLT} receives a Report message $r$, a Gate message $g$ is sent to the \ac{ONU} containing the grant size, which is calculate as the minimum between the requested window $r$ and the maximum allowed window $(W_{max})$.
%     
%     %To improve the \ac{QoS} provisioning, \ac{IPACT} can combine inter-ONU scheduling (centralize technique) to allocate the transmission windows to each ONU and a  priority queuing intra-\ac{ONU} scheduling (distributed technique) to divide the bandwidth allocated by the OLT among the different traffics  based on priorities or \ac{CoS} in the \ac{ONU}. %Finally, the adaptive cycle time is an important feature of \ac{IPACT}. Under saturation conditions, the cycle length is equal to the maximum cycle time, which will result in increased delay for all the packets. Under light loads, the cycle length decreases, resulting in more bandwidth being wasted by guard times and signaling. 
%
%    
%    %\commentc{Put info about QoS Intelligentce: Centrilized vs QoS Distributed}    
%
%%########################################################################
%% GIANT
%%########################################################################
%
%    %put here the references to the two alvaro's papers 
%    On the other hand, \ac{GIANT} is a well known \ac{DBA} algorithm for \ac{XGPON} \cite{Leligou_JCS2006_DAC:DAC761} that defines four type of bandwidths, namely, fixed, assured, non-assured and best-effort bandwidth. Alvarez \etal \cite{Pedro_NOC2014} \cite{Alvarez_JOCN2016-7444558} extends this algorithm to be used in \ac{XGPON}-based backhauling scenarios by introducing the \ac{gGIANT} algorithm. %. By adding a fifth type of bandwidth called group assured, \ac{gGIANT} allows 
%    This algorithm shares the assured bandwidth among multiple \acp{ONU} that serve base stations belonging to the same operator. The authors show the benefits of sharing the assured bandwidth among a group of base stations. Both algorithms, however, are based on the concept of centralized \ac{QoS} intelligence \cite{Stribling_CM2012_SIEPON_6295722}, in which the \ac{OLT} is the responsible for the \ac{QoS} provisioning of the individual queues at the \ac{ONU}. This is optimal for small business or individual users but not for users with multiple connections at each \ac{ONU} as in the mobile backhauling use case. 
%    
%   However, \ac{XGPON} has intrinsic features that make different of \ac{EPON}. \ac{GPON} have logical connections in the upstream and downstream direction called \ac{XGEM} ports to differentiate services which are established between \ac{OLT} and \ac{ONU}. Logical connections can also be grouped into \acp{T-CONT}. In this way, different levels of \ac{QoS} to different services belonging to a \ac{ONU} are enabled. A group \acp{T-CONT} into a single logical connection provide service to groups of \acp{ONU} called \ac{gT-CONT}, which is identified by the  \ac{gAllocId}. It means that some  \acp{T-CONT} of the same \ac{ONU} could be in different \ac{gT-CONT}. In contrast, \ac{EPON} technology do not use logical connections for different type of services because the \ac{ONU} realize the individual intra-scheduling for different type of traffic based on priorities and send just a packet with a size defined by the \ac{OLT}.
%
%\subsection{Policies for excess bandwidth distribution}
%\label{sec:excess-distribution}
%%the excess bandwidth algorithms in epon. 
%%5+ paper on excess distribution 
%% Novel bandwidth allocation with quota-based excess-distribution algorithm and wavelength assignment in multi-wavelength access network
%
%The first policy for excess bandwidth distribution was presented in \cite{EPON1}. %, where the wait-for-all-reports scheme was also introduced. 
%This policy, so called DBA1, takes advantage of statistical multiplexing to improve the network performance in a heterogeneous  scenario with \ac{BE}, \ac{AF}, and \ac{EF} traffic. % classes as defined in the \ac{DiffServ} framework. 
%It multiplies the excess bandwidth for the ratio between the REPORT of the \ac{ONU} target and the Total REPORTS of the all overload ONUs, thus it allocates the excess bandwidth according to the total demand of the overloaded ONU. This approach do not give an equal piece of the excess bandwidth for the overloaded ONUs because the bandwidth allocated depend of the individual request size.
%
%
%%It multiplies the excess bandwidth for the ratio between the REPORT of the ONU target  and the Total REPORTS of the all overload ONUs.
%%The DBA policy allocates the excess bandwidth according to the demand of the overload \acp{ONU} following \autoref{Ec:DBA1}.
%
%%  \begin{equation} 
%%  E_i = \frac{R_i}{\Sigma_{j\varepsilon %C}R_j}*E_{total}
%%  \label{Ec:DBA1}
%%  \centering 
%%  \end{equation}
%  
%%Where $C$ is the set of overloaded \acp{ONU} and $E_{total}$ the total excess bandwidth of all underloaded \acp{ONU} in a given scheduling cycle. This approach do not give an equal piece of the total excess because the excess allocated for a overloaded \ac{ONU} depend of the request size. 
%    
%A simple excess distributed policy, so called DBA2, was propsoed in \cite{EPON2}. It divides the total excess bandwidth $E_{total}$ equally among the overloaded \acp{ONU}. This kind of policy is known as uncontrolled excess because the \ac{OLT} allocates uniformly the excess to all overloaded \acp{ONU} regardless of the requested bandwidth by each ONU.  %The uncontrolled excess method do not consider the request size from \acp{ONU}, 
%This means that a overloaded \ac{ONU} can receive a grant larger than its buffer size. To avoid this problem, a controlled excess bandwidth policy (so called DBA3) was proposed in \cite{EPON3}. This avoids wasting resources by granting bandwidth less than or equal to the required ($G_i \leq R_i$). 
%%In the uncontrolled excess bandwidth algorithm, the GATE for a overload \ac{ONU} always is equivalent to the sum between the maximum transmission window size and the excess bandwidth $(G_i = W_{max} + E_i)$. However, in DBA3 when the REPORT is less than this value $(W_{max} + E_i)$, the GATE is equal to the REPORT. This way the system do not assign more resources to a overload \ac{ONU} that it does not need it. 
%
%%In DBA1 and DBA2, there are no an excess controlled, it means a GATE for a overload \ac{ONU} always is equivalent to the sum between the maximum transmission window size and the excess bandwidth $(G_i = W_{max} + E_i)$. However, in DBA3 when the REPORT is less than this value $(W_{max} + E_i)$, the GATE is equal to the REPORT. This way the system do not assign more resources to a overload \ac{ONU} that it does not need it. 
%
%%This approach gives an equal piece of the total excess for all ONUs, implying fairness. 
%        
%%    \begin{equation} 
%%    E_i = \frac{1}{M}*E_{total}
%%    \label{Ec:DBA2}
%%    \centering 
%%    \end{equation}
%    
%
%
%
%In \ac{EPON} network coexist several services, thus the $W_{max}$ could be different for all \acp{ONU}. The DBA1 and DBA3 algorithm, distributed the bandwidth only using the REPORT.  The problem with this approaches it that they assume the all ONUs are in the equal conditions. In a unbalanced scenario in which the ONU have difference guaranteed bit rates, the algorithms before mentioned produce unfairness. Other approach called WDBA was proposed in \cite{EPON4}. This algorithm realize a better fairness bandwidth distribution, due to use  of the bandwidth excess required $(B_{req} = Ri - W_{max})$ instead of just the REPORT. If is applies the controlled
%excess method, it leads a new algorithm called WDA1 \cite{EPON2}. 
%    
%    
%   %\begin{equation} 
%    %E_i = \frac{B_{i_{req}}}{\Sigma_{j\varepsilon C}B_{j_{req}}}*E_{total}
%   %\label{Ec:WBA}
%   %\centering 
%   %\end{equation}
%  
%
%\subsection{Summary}
%\label{sec:rw-summay}
%
%In summary, none of the above-reviewed \ac{EPON} \ac{DBA} schemes support group-\ac{SLA}. Even though there exists a \ac{XGPON} \ac{DBA} algorithm that supports group assured bandwidth, it cannot directly applied to \ac{EPON} networks. 
%First, \ac{XGPON} networks has a maximum cycle length of 125 us, whereas \ac{EPON} networks has a typical maximum cycle length value from 1 ms to 10 ms. This may help to improve the benefits the group \ac{SLA} concept brings since more bandwidth can be redistributed in a given scheduling period. Second, this paper works in a hierarchical DBA scheme in which the \ac{OLT} guarantees a given bandwidth while the intra-\ac{ONU} scheduler at the ONU is the responsible for providing the \ac{QoS} requirement of the different traffic \ac{ONU} flows. 
%
%
%

==> tabla.tex <==

\captionsetup[table]{skip=0pt}
\begin{table}[!t]
\caption{Simulation Parameters}
\label{tab:simulation-parameters}
\renewcommand{\arraystretch}{1.2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}||@{}c@{}}
\hline
\bfseries Parameter & \bfseries Value\\
\hline\hline
Optical link speed & 25 Gbps\\\hline
Upstream wavelength channels & 2\\\hline
PON capacity &  50 Gbps \\\hline
Maximum cycle length & 1 ms\\\hline
Guard band & 0.624 $\mu$s \\\hline
\begin{tabular}{c}Distance between OLT and ONUs\end{tabular} & \unit{[1,10] km}\\\hline
Propagation delay in fiber & 5 $\mu$s/km\\\hline
OLT-ONU RTT & \unit{[10,100] $\mu$s}\\\hline
ONU buffer size & 10 MB\\\hline
Total number of \acp{ONU} ($\left\vert\mathcal{O}\right\vert$) & 32\\\hline
\begin{tabular}{c}
Maximum available bandwidth for each  \\  ONU $(bw_i)$ \\
\end{tabular}
& 1.531 Gbps \\\hline
\begin{tabular}{c}Offered load for each ONU  $(\lambda_{i})$
\end{tabular} & $[0.6,1.0] \cdot bw_i$ \\\hline %\unit[0]{Mbps}$-$\unit[600]{Mbps} 
\ac{DWBA} algorithms  & 
\begin{tabular}{c} 
\BS  ($\theta=0.015$)%(\GSIPACT with  multi-\\thread and HPS distribution policy)
\\
\FLa and \FLb   %(Limited and Limited \\with excess distribution policy)
\end{tabular}
\\\hline
Intra-ONU scheduler & strict priority \\\hline
TWDW-PON architectures & 
\begin{tabular}{c} 
SSD,
MSD and
FF
\end{tabular}
\\\hline

\end{tabular}



}
%\vspace*{-1.5em}
\end{table}


==> web.tex <==
    \newcommand{\MYheader}{\smash{\scriptsize
    \hfil\parbox[t][\height][t]{\textwidth}{\centering {\normalsize
    To be published in the 54th IEEE International Conference on Communications (ICC 2020)}}\hfil\hbox{}}}
    \makeatletter
    % normal pages
    \def\ps@headings{%
    \def\@oddhead{\MYheader}
    \def\@evenhead{\MYheader}
    \def\@oddfoot{  }%
    \def\@evenfoot{  }}
    % title page
    \def\ps@IEEEtitlepagestyle{%
    \def\@oddhead{\MYheader}%
    \def\@evenhead{\MYheader}%
    \def\@oddfoot{   }%
    \def\@evenfoot{   }}
    \makeatother
    % make changes take effect
    \pagestyle{headings}
    % adjust as needed
    \addtolength{\footskip}{0\baselineskip}
    \addtolength{\textheight}{-0.1\baselineskip}
    
    
\normalem
